Reinforcement Learning Neural Turing Machines - Revised

The Neural Turing Machine (NTM) is more expressive than all previously considered models because of its external memory. It can be viewed as a broader effort to use abstract external Interfaces and to learn a parametric model that interacts with them. The capabilities of a model can be extended by providing it with proper Interfaces that interact with the world. These external Interfaces include memory, a database, a search engine, or a piece of software such as a theorem verifier. Some of these Interfaces are provided by the developers of the model. However, many important existing Interfaces, such as databases and search engines, are discrete. We examine feasibility of learning models to interact with discrete Interfaces. We investigate the following discrete Interfaces: a memory Tape, an input Tape, and an output Tape. We use a Reinforcement Learning algorithm to train a neural network that interacts with such Interfaces to solve simple algorithmic tasks. Our Interfaces are expressive enough to make our model Turing complete.

==> Makefile <==
PARTS=rlntm.tex

all: clean rlntm.pdf 

fast:
	pdflatex -shell-escape rlntm
	bibtex  rlntm	


rlntm.pdf: clean $(PARTS) rlntm.bib 
	pdflatex -shell-escape rlntm.tex 
	bibtex rlntm
	bibtex rlntm
	pdflatex -shell-escape rlntm.tex 
	pdflatex -shell-escape rlntm.tex 

clean:
	rm -f *.log *.blg *.aux *.bbl *.4tc *.xref *.tmp *.dvi *.hd *.idx *.out *.toc *.drv *.ins *.pdf
	rm -rf ~*
	rm -rf *.tmp
	rm -rf *.4om
	rm -rf *~
	rm -rf *.swp


tar:
	find . -type f | egrep -v '\.git|\.log|\.swp' | xargs tar zcvf ../rlntm.tar.gz




==> img/tree.tex <==
\begin{figure}
  \centering
  {
  \tiny
   \begingroup\makeatletter\def\f@size{1}\check@mathfonts
    \scalebox{0.75}{
    \begin{tikzpicture}
      \node [draw, circle] (r) at (0,0) {$r$};
      \node [draw, circle] (r0) at (-0.5,1) {$r_0$};
      \node [draw, circle] (r1) at (0.5,1) {$r_1$};
      \node [draw, circle] (r00) at (-1.5,2) {$r_{00}$};
      \node [draw, circle] (r01) at (-0.5,2) {$r_{01}$};
      \node [draw, circle] (r10) at (0.5,2) {$r_{10}$};
      \node [draw, circle] (r11) at (1.5,2) {$r_{11}$};
      \node [draw, circle] (r000) at (-3.5,3) {$r_{000}$};
      \node [draw, circle] (r001) at (-2.5,3) {$r_{001}$};
      \node [draw, circle] (r010) at (-1.5,3) {$r_{010}$};
      \node [draw, circle] (r011) at (-0.5,3) {$r_{011}$};
      \node [draw, circle] (r100) at (0.5,3) {$r_{100}$};
      \node [draw, circle] (r101) at (1.5,3) {$r_{101}$};
      \node [draw, circle] (r110) at (2.5,3) {$r_{110}$};
      \node [draw, circle] (r111) at (3.5,3) {$r_{111}$};
      \node [draw, circle] (r0000) at (-3.75,4) {$r_{\dots}$};
      \node [draw, circle] (r0001) at (-3.25,4) {$r_{\dots}$};
      \node [draw, circle] (r0010) at (-2.75,4) {$r_{\dots}$};
      \node [draw, circle] (r0011) at (-2.25,4) {$r_{\dots}$};
      \node [draw, circle] (r0100) at (-1.75,4) {$r_{\dots}$};
      \node [draw, circle] (r0101) at (-1.25,4) {$r_{\dots}$};
      \node [draw, circle] (r0110) at (-0.75,4) {$r_{\dots}$};
      \node [draw, circle] (r0111) at (-0.25,4) {$r_{\dots}$};
      \node [draw, circle] (r1000) at (0.25,4) {$r_{\dots}$};
      \node [draw, circle] (r1001) at (0.75,4) {$r_{\dots}$};
      \node [draw, circle] (r1010) at (1.25,4) {$r_{\dots}$};
      \node [draw, circle] (r1011) at (1.75,4) {$r_{\dots}$};
      \node [draw, circle] (r1100) at (2.25,4) {$r_{\dots}$};
      \node [draw, circle] (r1101) at (2.75,4) {$r_{\dots}$};
      \node [draw, circle] (r1110) at (3.25,4) {$r_{\dots}$};
      \node [draw, circle] (r1111) at (3.75,4) {$r_{\dots}$};

      \draw [thick] [->] (r) to (r0);
      \draw [dotted] [->] (r) to (r1);
      \draw [dotted] [->] (r0) to (r00);
      \draw [thick] [->] (r0) to (r01);
      \draw [dotted] [->] (r1) to (r10);
      \draw [dotted] [->] (r1) to (r11);
      \draw [dotted] [->] (r00) to (r000);
      \draw [dotted] [->] (r00) to (r001);
      \draw [dotted] [->] (r01) to (r010);
      \draw [thick] [->] (r01) to (r011);
      \draw [dotted] [->] (r10) to (r100);
      \draw [dotted] [->] (r10) to (r101);
      \draw [dotted] [->] (r11) to (r110);
      \draw [dotted] [->] (r11) to (r111);
      \draw [dotted] [->] (r000) to (r0000);
      \draw [dotted] [->] (r000) to (r0001);
      \draw [dotted] [->] (r001) to (r0010);
      \draw [dotted] [->] (r001) to (r0011);
      \draw [dotted] [->] (r010) to (r0100);
      \draw [dotted] [->] (r010) to (r0101);
      \draw [thick] [->] (r011) to (r0110);
      \draw [dotted] [->] (r011) to (r0111);
      \draw [dotted] [->] (r100) to (r1000);
      \draw [dotted] [->] (r100) to (r1001);
      \draw [dotted] [->] (r101) to (r1010);
      \draw [dotted] [->] (r101) to (r1011);
      \draw [dotted] [->] (r110) to (r1100);
      \draw [dotted] [->] (r110) to (r1101);
      \draw [dotted] [->] (r111) to (r1110);
      \draw [dotted] [->] (r111) to (r1111);
      \end{tikzpicture}
      }
      \endgroup
    }
  \caption{Tree of all possible actions. Every node has a reward. 
    {\it Reinforce} algorithm samples paths from such tree. Thick lines correspond
  to an exemplary sampled path. This sampled path yields a total reward: $r + r_0 + r_{01} + r_{011} + r_{0110}$.}
  \label{fig:tree}
\end{figure}



